Soothing Sensations: Enhancing Interactions with a Socially Assistive Robot through Vibrotactile Heartbeats

Physical interactions with socially assistive robots (SARs) positively affect user wellbeing. However, haptic experiences when touching a SAR are typically limited to perceiving the robot's movements or shell texture, while other modalities that could enhance the touch experience with the robot, such as vibrotactile stimulation, are under-explored. In this exploratory qualitative study, we investigate the potential of enhancing human interaction with the PARO robot through vibrotactile heartbeats, with the goal to regulate subjective wellbeing during stressful situations. We conducted in-depth one-on-one interviews with 30 participants, who watched three horror movie clips alone, with PARO, and with a PARO that displayed a vibrotactile heartbeat. Our findings show that PARO's presence and its interactive capabilities can help users regulate emotions through attentional redeployment from a stressor toward the robot. The vibrotactile heartbeat further reinforced PARO's physical and social presence, enhancing the socio-emotional support provided by the robot and its perceived life-likeness. We discuss the impact of individual differences in user experience and implications for the future design of life-like vibrotactile stimulation for SARs.

==> ChangeLog.tex <==

\section{Change Log from HRI 2024 Submission to Ro-man Submission}


\textbf{ Title: }
V0 : Heartfelt Companions: User Experiences with a Socially Assistive Robot that displays Vibrotactile Heartbeats

V1:  Soothing Sensations:  Enhancing Interaction with Socially Assistive Robots through Vibrotactile Heartbeats

V1*: Heartfelt Connections: Exploring User Experiences of a vibrotactile Heartbeat Display for Emotional Support in SARs

V1**: Heartfelt Companions: A qualitative exploration of User Experiences with a Socially Assistive Robot that displays Vibrotactile Heartbeats

\textbf{Abstract}
\begin{itemize}
    \item  clarified that study is qualitatitive
    \item ToDo: Improve implications statements
\end{itemize}
\textbf{Introduction }
\begin{itemize}
    \item to shorten paper, avoiding repetitions,  and to make the narrative more cohesive
    \item changed the contribution statements to be more clear and relevant to HRI community
\end{itemize}

\textbf{Methods}
\begin{itemize}
    \item added ethics statement
    \item added section on semi-structured interviews, to emphasise why we chose a qualitative over quantitative approach and providing a link to the full interview guide
    \item 
\end{itemize}

\textbf{Conclusions}
\begin{itemize}
    \item Rewrote the conclusion to make takeaways for HRI community clearer
    \item removed any statement regarding how findings are generalisable to a broader population
\end{itemize}

\textbf{Misc}
\begin{itemize}
    \item Removed any statement such as 'Authors in [1]' and replaced it with "citeauthor{1}". 
    \item removed any statement regarding how findings are generalisable to a broader population
\end{itemize}

